Understanding and Facilitating Mental Health Help-Seeking of Young Adults: A Socio-technical Ecosystem Framework

Prior research on young adults' mental health help-seeking mostly focuses on one particular resource such as a mobile app or digital platform, paying less attention to their lived experiences interacting with the ecosystem of resources. We conducted in-depth interviews with 18 participants about their help-seeking and non-help-seeking experiences. Guided by Social Ecological Theory, we proposed a Socio-technical Ecosystem Framework for mental health care, consisting of four levels of resources, including technological-, interpersonal-, community-, and societal level resources. Using this framework, we identified two types of support systems for help-seeking, single-resource support system and multi-resource support system. These resources support young adults' help-seeking via three mechanisms, \textit{care-giving}, \textit{care-mediating}, and \textit{care-outreaching}, forming various pathways to care. We then pointed out the barriers to resource use at each level and the general challenges in finding a support system. Our findings contributed to a conceptual framework to categorize mental health care. It also serves as a practical framework to identify challenges in the pathways to care and discover design implications.

==> cut.tex <==
Abstract
 We developed Andersen's health resource utilization model to identify factors that influence young adults' choice of resources and characterize their dynamic interactions with the socio-technical ecosystem. To find an appropriate support system, they recursively make efforts to interact with and obtain feedback from various resources. 
 
\section{lit review}
\subsection{low use of technology}
%For example, Stawarz et al. \cite{stawarz_use_2019} found that certain apps guided activities and enabled tracking, while social media served as sources of learning peer experiences and websites offer insights into how to deal with day-to-day basis stress. 

%Beyond lab experiments and user tests with a small number, larger survey studies found that the acceptance and utilization of these technologies are still limited in the real world, especially for people with low technology literacy or socioeconomic status. Eccles et al. noticed that some people explicitly expressed an aversion to using the Internet to prevent mental health \cite{h_barriers_2021}. Some studies in rural settings found that farmers and villages are not interested in using technology-based services (e.g., digital platforms \cite{c_dont_2021} and SMS referral systems \cite{a_lessons_2020}) because of the low benefit. Other studies pointed out challenges in difficulties in finding appropriate mobile apps \cite{n_finding_2015}. Other difficulties involved in using technologies included low adjustability, usability, trustworthiness, and privacy protection \cite{geerling_why_2023} and confusion, leading to inaccurate self-diagnosis, or ambiguous and overloading \cite{pendse_mental_2019, c_profiling_2022, pretorius_young_2019}.

\subsection{Resource Pathways to Care}
To understand how participants interact with resources at different levels in the socio-technical ecosystem for mental health help-seeking, we depicted various pathways to care, including professional, informal, and self help. Each resource may offer different functions, including care-giving, care-mediating, and care-outreaching. Care-giving means that a resource offers people informational, emotional, clinical, or financial support. Care-mediating means that a resource acts as a bridge between one resource and the other. Care-outreaching means that a resource actively reaches out to potential users to provide help, such as services that directly intervene when certain situations emerge.

\subsubsection{Technology-mediated pathways} Fig \ref{fig:technology} shows the pathways to care through technologies. Technologies serve as care-giving and care-mediating in the three pathways. 

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/Technology2.jpg}
    \caption{Technology-level pathways}
    \label{fig:technology}
\end{figure}

Technology: Care-giving. Participants mostly got informational support from online information from search engines, online forums, and video-sharing platforms. 

Technology: Care-mediating. 

\textbf{Self->Search Engines/Webpages->Professionals/online forums (T1)}. Some participants, demonstrated by T1-a in Figure 3, directly sought answers related to symptoms, potential causes, and guidance on how to cope with mental distress using search engines and websites. Some participants (shown by T1-b) followed the lead of online information to access professionals. For example, three participants (P01, P08, and P13) mentioned using the Psychological Today website to look for therapists that fit their preferences on factors such as gender, education, location, and cost. Sometimes, search engines and websites' mediating effects take place over time by gradually changing participants' knowledge and understanding of professional help. For instance, P07 decided to explore medication as a potential solution after repeatedly encountering recommendations from Google search results.

\textbf{Self->Online Communities (T2)}. Some participants aimed to obtain support and understanding directly from online communities (T2-a). They read other people's stories, commented on posts, and shared their own experiences. P05 and P18 considered "online friends" even better than their "real friends." P12 explained, "\textit{I will say this online group is safer because the online friends have seen their issues but, the majority of my physical friends don't experience what I'm experiencing. }"
Some participants developed interpersonal relationships within online groups (T2-b). For instance, P02 formed connections with two online friends through Facebook groups and frequently shared recent experiences with them.

\textbf{Self->Video Sharing/Gaming Platforms (T3)} served as a way to "distract" people from mental health concerns. Among the participants, P03 intentionally immersed herself in TikTok videos to relax and P13 watched YouTube videos to escape from mental health worries. P13 commented, "\textit{People, laughing, banter, escapism... I think distraction is actually a very important way, at least to amuse ourselves and just to get rid of the stress from life.} "

\subsubsection{Interpersonal-level pathway} Interpersonal relationships contain the most natural sources of help- blood and social relationships, typically family and friends. 
Figure \ref{fig:Interpersonal} shows the pathways at this level.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/Interpersonal2.jpg}
    \caption{Interpersonal-level pathways}
    \label{fig:Interpersonal}
\end{figure}

1. Self-> family/friends (family/friends as a care-giving source)
2. Self->family/friends ->Professionals (family/friends as a care-mediating source)
3. Family/friends ->Self->Professionals (family/friends as a care-outreaching source)

\textbf{Family/Friends-Self-Professional (I1)} was mentioned by five participants. Family and friends play a crucial role in identifying early-stage symptoms due to their daily interactions with the individuals. For example, P16, who locked herself at home for two months following her mother's passing without realizing she might have depression, had friends who constantly checked on her and eventually took her to the hospital. She expressed gratitude for their intervention, stating, "\textit{This was too much for me.  They came in when I lost it during that time. They took me to the hospital, checked with the hospital, and showed that I really needed this [professional help]. }"

\textbf{Self-Family/Friends->Professional (I2).} Six participants openly shared their mental distress with interpersonal relationships (I2-a) and sought emotional, financial, and informational support to access professional help (I2-b). Participants' family and friends recommended mental health resources, including therapists and hotlines (P13, P18), covered treatment costs (P02, P04), and provided encouragement for ongoing treatment (P12, P14).

\textbf{Self-Family/Friends (I3)} provides direct emotional support without necessitating disclosure of mental distress. P14 expressed confidence that "\textit{Obviously they're [my friends] gonna support me,}" although "\textit{actually I don't want to tell my mental distress.}" Some participants found solace in the companionship of family and friends, using it as a substitute for professional help. For instance, P18 mentioned that "\textit{she came with immediate effects. She encouraged me, talked to me, and we played games.}"

\subsubsection{Community-level pathway} Community mental health resources were primarily accessible within educational institutions, including schools and universities. While P13, a sports official, noted that stress management training was offered by his employer, workplace-based mental health support was relatively limited. Other community settings such as residential areas and commercial companies demonstrated lesser investment in mental health services.
Fig \ref{fig:Community} shows the pathways at this level. 

\begin{figure} [h]
    \centering
    \includegraphics[width=\linewidth]{images/Community2.jpg}
    \caption{Community-level pathways and Societal-level pathways}
    \label{fig:Community}
\end{figure}

%preliminary, middle, and high schools. Before university, many schools do not set up an independent department with professionals in mental health, thus teacher is an available source perceived by adolescents. 

1. Self->Community services (community services as a care-giving source)
2. Self->community services ->professionals (care-mediating)
3. Community services->self (care-outreaching)

\textbf{Self-Community services (C1)} were utilized by eight participants. 
Certain universities proactively engage with their communities (C1-a) by disseminating information and resources through diverse channels, including emails, social media platforms, and awareness events. P10 and P13 noted the pervasive presence of university hotline signs in hallways, offices, and dining halls. 
Within university settings, community mental health support was effectively integrated with other accommodations (C1-b). P06 requested a reduced class load, P07 received extended tuition payment options, and P08 benefited from continued free therapy sessions post-graduation. They heavily relied on universities' free resources (e.g., psychiatry visits and free therapy sessions).
%P07 shared her experience seeking help from one of her teachers, "\textit{I remember I cried to her about how I was feeling, and it was just nice to let someone at school know how it's feeling. I felt like I could breathe better with her knowing.}" 

\subsubsection{Societal-level pathway}
%includes access to professional help through national lifeline, governmental institutions, and non-governmental organizations.
%Direct pathway to care illustrated that participants got in touch with professional mental health services directly, including hierarchical institutions and health workers such as hospitals, clinics, psychiatrists, therapists, nurses, etc. 
No participants directly accessed professional help, or successfully used governmental institutions or non-governmental organizations to access professional help. The barriers in such pathways are discussed in Sec 5.
1. self->national lifeline (as a caregiving source)
2. Self->national lifeline -> professionals (as a mediating source)
3. lifeline -> self (lifeline as a care-outreaching source)

\textbf{Self-National Lifeline-Professionals (S1)} was mentioned by several participants as a channel to turn to in an emergency (S1-a, shown in Fig \ref{fig:Community}). P07 called this lifeline after she cut herself but her therapist was unavailable. She commented, "\textit{I just wanted to talk to someone that would listen to me... I think I got what I needed out of it, like just talking to someone because it was able to calm me down quite a bit.}" In some occasions, calling the Lifeline can result in mandatory hospitalization (S1-b). P14 was afraid to use the Lifeline because her friend was placed in hospital after calling.
%Some participants mentioned their and others' bad experiences with Lifeline because of its limited availability, certain mandatory policies, and disappointing responses. 
%P14 called Lifeline in 2018 which put her on hold for two hours and did not go through. P13 was discouraged by the staff who answered his call because "\textit{I wasn't really actively suicidal right then, but I was very much considering it, so I called it. When they realized that I wasn't actively trying to do something, they kind of seem to more blow me off, as if oh everyone has bad days, yeah, you're depressed, but you know, other people have it worse. And I was like, oh, okay. Thank you.}" 

\subsubsection{Multiple-level pathway} \label{para: multi} We identified two pathways that involve close collaborations among multiple levels of resources.
\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{images/multiple.jpg}
    \caption{Multiple-level pathways}
    \label{fig:multiple}
\end{figure}
How to further abstract the pathways below? they are very empirical. 
community -> interpersonal -> self -> professional 
self->community hotlines->community coordinators -> professional <should this belong to self->community sources->professionals, given both hotlines and coordinators are community sources>

\textbf{Community-Parents-Self-Professionals (M1).} Teachers played a pivotal role in recognizing and engaging parents in addressing mental health symptoms during participants' youth. For three participants, teachers identified signs of mental health issues and informed their parents, leading to professional intervention. In addition to notifying parents, teachers monitored participants' recovery and facilitated timely information exchange with parents.
%"\textit{In senior year of high school, they [suicidal thoughts] got really bad and I went to see one of the counselors.}" 

\textbf{Self-Community Hotlines-Community Coordinators-Professionals (M2)} illustrates the effectiveness of the community in responding to emergencies. P07 called the university crisis line to request accommodations. Upon learning about her self-harm tendencies, the staff dispatched a police officer and a doctor to her residence. They escorted her to a local hospital, where she was diagnosed with major depressive disorder and generalized anxiety disorder and got medications, as she recounted,"\textit{I stayed in the hospital for two days..they diagnosed me with a major depressive disorder and generalized anxiety disorder, and then that's when they gave me a medication to start to treat both of those.}"


\section{RQ2: What characteristics are valued in young adults' mental health help-seeking?}
\subsection{Enabling affordances of each level of resources.}
Driven by the need to seek help, participants evaluated the enabling affordances of resources to determine their preferred points of contact.
Anderson's model \cite{andersen_revisiting_1995} did not provide specific factors affecting resource choice, we identify distinct characteristics that facilitate or impede resource access, including availability, safety, support, and sustainability affordances (in Tab \ref{fig:enabling}).

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{images/enabling.png}
    \caption{Enabling Factors}
    \label{fig:enabling}
\end{figure}

\subsubsection{Availability}
and safety are keys to encouraging participants to consult in first contact with resources, especially for participants who have suppressed their needs for a long time. In urgent situations, technology and community resources were mostly chosen by participants. 
Technology is the most available and anonymous resource with on-demand and 24/7 access to online information. P12 thought \pquote{The most helpful is social media because you can go on it anytime. There's always someone on the group to read and give you your answer.} and \pquote{.. this online group is safer because they have seen what I have seen. My physical friends, the majority of them don't experience what I'm experiencing.}
The community resources are located in the environment young people are living in and university resources are usually inexpensive or even free, so they are perceived to be easier to access. P04 recalled he went to the university MH center, \pquote{Because I felt I could not handle it alone anymore and they were the closest and had anonymity.} He further explained that 
\pquote{They contact your department or your parents, only in cases of emergency. But besides that, everything that you come in and say is kept confidential.}
Despite technologies are not personalized and interactive enough for some participants, they act as security guards when other help is unavailable. For example, the therapist and a great friend,
In urgent scenarios: Technologies provide a way to societal backup. 

\subsubsection{Safety}
 affordances vary among participants.
Individual differences influence the interpretation of the same resource. P05 suspects the anonymity of online forums because \pquote{I feel like these people around me might have an ICA spying on me. So, I felt there was a pushback that prevented me from writing my experiences in online groups.}
Participants appreciated the privacy and availability technology affords, for example, P13 said \pquote{Technology could let no one else know that you search this information. I think it's so much easier to not have to try and ask other people... I don't want no people to know. So it's much easier to find stuff online.}
Accommodation policies can boost safety by providing academic and performance. 

\textbf{Care-outreaching: Comprehensive and sustainable support.} Interpersonal relationships can offer emotional, information, and financial support, which provide a strong base for seeking professional help. <> Interpersonal support is sustainable over time and across locations. Communication technologies further strengthen the stability and continuity of interpersonal relationships in the face of external changes such as moving. <>
Interactions with interpersonal relationships are a natural part of young adults' everyday lives, giving them the ideal position to identify symptoms. Among XX participants who used interpersonal resources, XX of their symptoms was first identified by parents/friends. \pquote{I did not want, as I said, to associate with anyone, just wanted to be myself to be alone...When I lost it during that time, they took me to the hospital. They helped me. If you have the right support system, this support system can help you come around and make you realize that you need this. So, by checking with the hospital. And that showed that I really needed this.} (P16)
\pquote{Like in our building, it's all over the place. I can see it in an elevator, and even in our office. I know the crisis line.} (P10)
\subsubsection{Support}
\textbf{Active and comprehensive care-outreaching.} Many participants pointed out that they were aware of the university mental health center because it actively reaches out to students. 

P07 and P08 were almost passively dragged out by policy infrastructure of mental health intervention (university hotline and awareness newsletter)- Actively reaching out is important; policy design about a trigger to force external assistance under certain circumstances). However, in P05's case, when that program knew about the crime-related post-traumatic anxiety and depression, there was no active involvement from the college, and he had to rely on his family resources, who finally had to send him to another place and drop out of college.

\subsubsection{Sustainability}
Opportunities of informal help-seeking. However, to still get emotional support, some participants tried to hang out with friends without explicitly disclosing their real mental status (P09, P10, P03). 
%emotional help and get the reassurance that <> "It is normal to have such issues". In the following interactions, participants would consider more clinical treatment efficacy and sustainability.

%\pquote{I wouldn't wanna discuss with someone whom I tend to know in person. Or because this looks like an anonymous kind of session.} (P17)

%\textbf{Availability of resources} is to what extent a resource can be easily accessed. Cost of time and money and resource delivery are two main determinants of availability. 
%The availability of interpersonal- and community-level depends on participants' specific contexts (e.g., relationships with family and friends, types of community). Among the twelve participants, six participants' families or friends are unavailable because of family issues (i.e., P05 was abandoned by divorced parents, P07's parents were too busy, P08's parents ignored her symptoms, and both P16's parents passed away) and lack of friends. 
%The societal-level resources are theoretically available to everyone, but in practice, it is participants' last choice since it costs a huge amount of time and money.

%Although interpersonal resources are generally unprofessional and informal, they perceived these resources as comfortable, reliable, and trustworthy. 
%\textbf{Policy} includes behavioral guidelines that regulate actions and feedback to a help-seeker. 
%Technology-level resources do not have any accommodations or mandatory policies but have the most strong protection of privacy. <P13> 
%Without written policies at interpersonal-level resources, feedback, and reactions from family and friends vary case by case. The families of P05 offered sufficient accommodations after knowing their symptoms and helped them move into new environments. Four participants (P07, P13, P14, P16) mentioned their interpersonal relationships took mandatory actions that forced them to be diagnosed and hospitalized. Participants had different attitudes toward these mandatory 
%Community-level resources were able to provide accommodations and conduct mandatory actions when necessary. Academic and work performance accommodations are important reassurances that facilitate help-seeking from community resources.
%Societal-level resources have the most standard regulations. Participants can theoretically trade accommodations by giving up part of their privacy. Sometimes, mandatory actions can also hurt participants' privacy needs.

%\textbf{Support} denotes clinical, informational, and emotional help provided by resources. Only formal mental health service providers (e.g., medical system, therapist, etc.) and some professional community resources (e.g., certified counselors) can provide clinical support. 
%Informational needs can be better supported by community- and societal-level resources in terms of professionality.
%Interpersonal-level resources were ideal sources for emotional support and technologies such as online communities can also provide emotional support.
%Sustainability means how long certain support can be stably supported, which is critical for mental health help-seeking. Community resources were generally temporary but interpersonal and societal resources can support long-term needs. The use of technology 

%\textbf{Sustainability Affordances} Community resources are temporary and transitional in nature, acting as a bridge between community members and the formal mental health care system, and are not available after the loss of membership (e.g., graduation, moving).

\subsection{Affordances}
\subsubsection{Agency \& mandatory}
\textbf{Authority of communities creates barriers.} 
In contrast, enforcement policies sometimes scare participants away. P14 didn't want to call the National Crisis Line because one friend was forced to a mental hospital after calling. She thought \pquote{that's like a big fear, at least with a lot of people that have depression or feeling suicidal, they're scared of that.}

Enhancing trust in mandatory practices. reported tensions and even hostile relationships between caregivers and patients, Based on the theoretical model– cognitive model of caregiving (Kuipers, Onwumere, \& Bebbington, 2010), which hinders patients from confiding in the carer and denying problems. 
Seeking help is a willingness to handle out part of autonomy, which allows other authority to make decisions for oneself or influence the decisions by oneself. There is an asymmetry in power, which could be a good thing for some participants so that they can get immediate attention and treatment, but it is probably bad for others because their privacy is offended and they would not trust this source again. 
P07 stopped going to the therapist and went back as the situation got worse. When she called the university crisis line to talk it out and get accommodations for her class registration, the coordinator sent 2 cops and 1 counselor to her apartment. The counselor came and convinced her to go to the hospital for an overnight stay. She came with the expectation to stay just one night but they forced her to stay two days. Although she was unhappy and unwilling to stay at the hospital at that time, looking back, she was happy that they intervened because \pquote{they know what they are doing.}

==> tables/crosstable.tex <==
% \usepackage{color}
% \usepackage{tabularray}
\definecolor{Black}{rgb}{0,0,0}
\definecolor{Silver}{rgb}{0.8,0.8,0.8}
\begin{table*}[h]
\centering
\sloppy
\hyphenpenalty 10000
\small
\caption{A framework of research agenda}
\label{tab:implications}
\begin{tblr}{
  width = \textwidth,
  % colsep = 1px,
  colspec = {|Q[r,0.5]|Q[l,1]|Q[l,1]|Q[l,1]|},
  % cell{1}{1} = {c=2}{c},
  % cell{1}{3} = {c=2}{c},
  % cell{1}{5} = {c=2}{c},
  hlines, %vlines,
  row{1} = {font=\bfseries,c,gray9},
  % row{2-4,6-8} = {ht=3.0\parskip}, % not work
}
  & Care-giving & Care-mediating & Care-outreaching \\
        Societal & Improving access rate  & Crisis line and emergency & Public health communication \\
        Community & Community service provision & Collaboration with professionals & Community communication and intervention \\
        Interpersonal &  & Collaborative   & Collaborative\\
        Technological & Self-management tools &  & Active monitoring tools\\
\end{tblr}
\end{table*}
